Calibration and Uncertainty Characterization for Ultra-Wideband Two-Way-Ranging Measurements

Ultra-Wideband (UWB) systems are becoming increasingly popular for indoor localization, where range measurements are obtained by measuring the time-of-flight of radio signals. However, the range measurements typically suffer from a systematic error or bias that must be corrected for high-accuracy localization. In this paper, a ranging protocol is proposed alongside a robust and scalable antenna-delay calibration procedure to accurately and efficiently calibrate antenna delays for many UWB tags. Additionally, the bias and uncertainty of the measurements are modelled as a function of the received-signal power. The full calibration procedure is presented using experimental training data of 3 aerial robots fitted with 2 UWB tags each, and then evaluated on 2 test experiments. A localization problem is then formulated on the experimental test data, and the calibrated measurements and their modelled uncertainty are fed into an extended Kalman filter (EKF). The proposed calibration is shown to yield an average of 46% improvement in localization accuracy. Lastly, the paper is accompanied by an open-source UWB-calibration Python library, which can be found at https://github.com/decargroup/uwb_calibration.

==> sections/optimal_delay.tex <==
\textcolor{red}{maybe show experimentally on transmit-receive-transmit} \\
\textcolor{red}{maybe add dynamic experiments?} \\
\textcolor{red}{note that were some changes that should be merged from ranging\_protocol.tex, especially after (2) and in subsection A} 

UWB ranging relies on the time-of-flight (ToF) of signals in order to compute range measurements. The simplest way to do this is using SS-TWR, shown in Figure~\ref{fig:ss_twr}, where the ToF measurement can be computed as 
\beq
\label{eq:ss_twr}
   t_\mathrm{f} = \f{1}{2} (\Delta t_{41} - \Delta t_{32}).
\eeq
However, different UWB tags have differrent clocks that are typically running at different rates, and this clock skew results in additional bias in the computed ToF measurement as will be shown below. In \cite{Neirynck2017}, an alternative DS-TWR-based ranging protocol is proposed to mitigate clock-skew-dependent bias. In this paper, the DS-TWR protocol shown in Figure~\ref{fig:ds_twr} is proposed, where the ToF measurement can then be computed as 
\beq
   \label{eq:ds_twr}
   t_\mathrm{f} = \f{1}{2} \left(\Delta t_{41} - \f{\Delta t_{64}}{\Delta t_{53}} \Delta t_{32} \right).
\eeq
This is slightly different than what is proposed in \cite{Neirynck2017}, and allows intuitively understanding the purpose of the additional response signal as further addressed later in this section. Additionally, this allows the device connected to the initiating tag to be the one that processes the range measurement.   

\subsection{Analytical Bias Model} \label{subsec:analyital_bias_model}

The two intervals in \eqref{eq:ss_twr} are of different time units due to the differing clock rates of the two tags, which consequently results in a clock-skew-dependent bias \cite{Neirynck2017}. To demonstrate this, consider in SS-TWR the clock-skew-corrupted time-of-flight measurement,
\beq
   \hat{t}_\mathrm{f}^\mathrm{ss} = \f{1}{2} \left( (1+\gamma_1) (\Delta t_{41} + \eta_4 - \eta_1) - (1+\gamma_2) (\Delta t_{32} + \eta_3 - \eta_2)  \right),
\eeq
where $\gamma_i$ is the skew of Tag $i$'s clock relative to an arbitrary global clock, $\eta_i \sim \mathcal{N}(0,R)$ is timestamping white noise associated with timestamp $t_i$, and $\eta_i$ and $\eta_j$ are mutually independent. From now onwards, the notational simplification $\eta_{ij} \triangleq \eta_i - \eta_j$ will be used. The ToF error is thus
\begin{align}
   e^\mathrm{ss} &\triangleq \hat{t}_\mathrm{f}^\mathrm{ss} - t_\mathrm{f} \\
   %
   &= \f{1}{2} \left( \gamma_1 \Delta t_{41} + (1+\gamma_1) \eta_{41} - \gamma_2 \Delta t_{32} - (1+\gamma_2) \eta_{32} \right), \label{eq:e_ss}
\end{align}
and the expected value of $e^\mathrm{ss}$ is  
\begin{align}
   \mathbb{E} \left[ e^\mathrm{ss} \right] &= \f{1}{2} \left( \gamma_1 \Delta t_{41} - \gamma_2 \Delta t_{32} \right) \label{eq:ss_mean_1}\\
   &\stackrel{\eqref{eq:ss_twr}}{=} \f{1}{2} \left( \gamma_1 (2 t_\mathrm{f} + \Delta t_{32}) - \gamma_2 \Delta t_{32} \right) \\
   &= \gamma_1 t_\mathrm{f} + \f{1}{2} \left( \gamma_1  - \gamma_2 \right) \Delta t_{32}. \label{eq:ss_mean}
\end{align}

The first component of \eqref{eq:ss_mean} is negligible as skew is usually in the order of parts-per-million and ToF in nanoseconds. However, $\Delta t_{32}$ is typically in hundreds or thousands of microseconds, meaning that clock-skew-dependent bias is not negligible. 

The correcting factor in \eqref{eq:ds_twr} consequently transforms $\Delta t_{32}$ from time units of Tag 2's clock to time units of Tag 1's clock. Rewriting \eqref{eq:ds_twr} as
\begin{align}
   t_\mathrm{f} = \f{\Delta t_{41}\Delta t_{53} - \Delta t_{64}\Delta t_{32}}{2 \Delta t_{53}}
\end{align}
and following the same steps as before, the ToF error for the proposed DS-TWR can be derived to be approximately
\begin{align}
   e^\mathrm{ds} &\triangleq \hat{t}_\mathrm{f}^\mathrm{ds} - t_\mathrm{f} \\
   &\approx \f{1}{2} \gamma_1 t_\mathrm{f} + \f{1}{2} \left( 1 + \gamma_1 \right) \left[ \f{\Delta t_{32}}{\Delta t_{53}} (\eta_{53} + \eta_{64}) + \eta_{41} + \eta_{23} \right],  \label{eq:e_ds}
\end{align}
where $\hat{t}_\mathrm{f}^\mathrm{ds}$ is the clock-skew-corrupted time-of-flight measurement. Deriving \eqref{eq:e_ds} relies on the assumption that
\begin{align}
   \Delta t_{53} \gg \norm{\eta_{53}}, \qquad \Delta t_{32} \gg \norm{\eta_{32}}.
\end{align}
This is expected since the timestamping error is typically in the order of nanoseconds, and the delay intervals are in the order of hundreds of microseconds. The expected value of the error is therefore
\begin{align}
   \mathbb{E} \left[ e^\mathrm{ds} \right] = \f{1}{2} \gamma_1 t_\mathrm{f}, \label{eq:ds_mean}
\end{align}
which suffers from less bias when compared to the error of the SS-TWR protocol.

\subsection{Analytical Variance Model}

Having addressed the accuracy of the measurements for SS-TWR and DS-TWR, it might appear that DS-TWR should always be used. However, the precision or variance of the measurements has not been addressed by \cite{Neirynck2017}. This is of particular importance in estimation and filtering applications, as noisy measurements increase uncertainty in the computed estimates thus consequently affect the ability to implement guidance and control algorithms.

Revisiting \eqref{eq:e_ss} and \eqref{eq:ss_mean_1}, the variance of the SS-TWR measurements is
\begin{align}
   &\mathbb{E} \left[ \left(e^\mathrm{ss} - \mathbb{E}[e^\mathrm{ss}]\right)^2 \right] \\ &= \mathbb{E} \left[ \left(\f{1}{2} \left((1+\gamma_1)\eta_{41} - (1+\gamma_2)\eta_{32} \right) \right)^2 \right] \\
   %
   &= R + \f{1}{2} (\gamma_1 + \gamma_2) R. \label{eq:var_ss}
\end{align} 
Similarly, by revisiting \eqref{eq:e_ds} and \eqref{eq:ds_mean}, the variance of the DS-TWR measurements is 
\begin{align}
   &\mathbb{E} \left[ \left(e^\mathrm{ds} - \mathbb{E}[e^\mathrm{ds}]\right)^2 \right] \\ &= \mathbb{E} \left[ \left( \f{1}{2} \left( 1 + \gamma_1 \right) \left[ \f{\Delta t_{32}}{\Delta t_{53}} (\eta_{53} + \eta_{64}) + \eta_{41} + \eta_{23} \right] \right)^2 \right] \\
   %
   &= (1+\gamma_1)^2 R + (1+\gamma_1)^2 \left( \f{\Delta t_{32}}{\Delta t_{53}} \right) R + (1+\gamma_1)^2 \left( \f{\Delta t_{32}}{\Delta t_{53}} \right)^2 R, \label{eq:var_ds}
\end{align}

Therefore, in the absence of clock skew (i.e., when $\gamma_1 = \gamma_2 = 0$), the variance of DS-TWR measurements is typically higher than SS-TWR measurements, and approaches the variance of SS-TWR as $\Delta t_{32} \to 0$ and/or $\Delta t_{53} \to \infty$. The former is due to the effect of the length of $\Delta t_{32}$ on the bias as discussed in Section~\ref{subsec:analyital_bias_model}, and the latter is due to the fact that the ratio $\f{\Delta t_{64}}{\Delta t_{53}}$ is being used to obtain a clock-skew measurement, and the longer the $\Delta t_{53}$ interval is the higher the signal-to-timestamping-noise ratio.

\subsection{Finding the Optimal Second-Response Delay}

Given \eqref{eq:var_ds}, minimizing $\Delta t_{32}$ is an obvious choice to reduce the variance of the measurements. However, it is less clear what is the right choice with $\Delta t_{53}$, as maximizing this second-response delay reduces measurement uncertainty but also reduces the frequency in which measurements are available. The choice of $\Delta t_{53}$ is thus application-specific. Most commonly in estimation applications, the goal is to minimize the uncertainty of the estimates which is achieved by maximizing the information attained from measurements. Therefore, this section poses an information-maximizing (variance-minimizing) optimization problem. 

The amount of \emph{information} attained in one unit of time is a function of two variables, 
\begin{enumerate}
    \item the uncertainty of the individual measurement, and
    \item the number of measurements in that unit of time. 
\end{enumerate}
As per \eqref{eq:var_ds}, the uncertainty in the individual measurement decreases as the delay in the second response (i.e., $\Delta t_{53}$, hereinafter referred to as \emph{the delay}) increases. However, as the delay increases, measurements occur less frequently, hence reducing the amount of information conveyed in a unit of time. As a result, the \emph{optimal} delay is one that is long enough to reduce the uncertainty of the individual measurement but short enough to ensure measurements are recorded at a sufficient frequency. 

Rewriting \eqref{eq:var_ds} in the absence of clock skews yields
\beq
    R_i \triangleq R + \f{\Delta t_{32}}{\Delta t_{53}} R + \left(\f{\Delta t_{32}}{\Delta t_{53}}\right)^2 R,
\eeq
for the individual measurement. The time-length of one measurement can be defined to be $T + \Delta t_{53}$ seconds long, where the time taken for all other signals and computational processing is lumped into the $T$ term as $\Delta t_{53}$ is the only variable of concern. Therefore, in one second, a total of $\f{1}{T + \Delta t_{53}}$ measurements occur, meaning that the overall uncertainty (inverse of information) of the measurements is given as
\begin{align}
    R_\mathrm{tot} &\triangleq (T + \Delta t_{53}) R_i \\
    %
    &= R \left[(T + \Delta t_{53}) + \f{\Delta t_{32} (T + \Delta t_{53})}{\Delta t_{53}} + \f{(\Delta t_{32})^2(T + \Delta t_{53})}{(\Delta t_{53})^2}\right]. \label{eq:Rt}
\end{align}
%
The derivative of \eqref{eq:Rt} w.r.t. $\Delta t_{53}$ is then
\beq
    \f{\dee R_\mathrm{tot}}{\dee \Delta t_{53}} = R - T \f{\Delta t_{32}}{(\Delta t_{53})^{2}} R - 2T \f{(\Delta t_{32})^2}{(\Delta t_{53})^{3}} R - \f{(\Delta t_{32})^2}{(\Delta t_{53})^{2}} R,
\eeq
and equating to 0 yields
\begin{align}
    0 &= (\Delta t_{53})^3 - \Delta t_{32} (T + \Delta t_{32}) \Delta t_{53} - 2(\Delta t_{32})^2 T. \label{eq:optimal_delay}
\end{align}

The value for $T$ and $\Delta t_{32}$ can be determined experimentally and are both processor and application dependent. As an example where $T=4.5$ ms and $\Delta t_{32}=0.3$ ms, the optimal delay can be found analytically to be approximately 1420 $\mu$s using \eqref{eq:optimal_delay}. This is also shown in Figure~\ref{fig:optimal_delay}.

\begin{figure}
   \includegraphics[trim={8cm 0cm 8cm 0cm},width=\columnwidth]{figs/optimal_delay/optimal_delay.pdf}
   \caption{\textcolor{red}{Should I keep this? If so, need to make similar changes to Fig 4. If removed, need to make corresponding changes in text}}
   \label{fig:optimal_delay}
\end{figure}

\subsection{Experimental Results}

\begin{figure}[t!]
   \centering
   \begin{subfigure}[t]{0.4\columnwidth}
       \centering
       \includegraphics[trim={11cm 0cm 11cm 0cm},width=\columnwidth]{figs/misc/ourboard_compressed.png}
       \caption{Custom-made board fitted with DWM1000 UWB transceivers.}
       \label{fig:uwb_board}
   \end{subfigure}%
   ~ \hspace{5pt}
   \begin{subfigure}[t]{0.55\columnwidth}
      \centering
      \includegraphics[width=\columnwidth]{figs/optimal_delay/IMG_0779.jpg}
      \caption{Two static tripods each fitted with a UWB tag.}
      \label{fig:optimal_delay_experiment}
  \end{subfigure}%
   \caption{Experimental set-up for studying the effect of $\Delta t_{53}$ in DS-TWR on the variance of the measurements.}
\end{figure}

\begin{figure}[t!]
   \centering
   \begin{subfigure}[t]{\columnwidth}
      \centering
      \includegraphics[trim={6cm 2cm 6cm 0cm},width=\columnwidth]{figs/optimal_delay/2022_08_05_optimal_delay_metrics.pdf}
      \caption{$\Delta t_{32} = 300$ $\mu$s.}
      \label{fig:optimal_delay_metrics}
   \end{subfigure}%
   \\ \vspace{5pt}
   \begin{subfigure}[t]{\columnwidth}
      \centering
      \includegraphics[trim={6cm 0cm 6cm 0cm},width=\columnwidth]{figs/optimal_delay/2022_08_09_optimal_delay_d1_1500_metrics.pdf}
      \caption{$\Delta t_{32} = 1500$ $\mu$s.}
      \label{fig:optimal_delay_metrics_1500}
   \end{subfigure}
   \caption{\textcolor{red}{1) add line or something at minimum}. \textcolor{red}{2) change x-axis to be delta 53. 3) make Rt to Rmathrmtot} Scatter plot showing the effect of $\Delta t_{53}$ on $R_\mathrm{tot}$, the standard deviation of the measurements, and the frequency in which measurements are recorded.}
\end{figure}

To evaluate the effect of the second-response delay $\Delta t_{53}$ on a real system, the following experiment is set up. Two custom-made boards shown in Figure~\ref{fig:uwb_board} equipped with DWM1000 UWB transceivers \cite{dw1000} are fixed to two static tripods as shown in Figure~\ref{fig:optimal_delay_experiment}. They are both connected to a Dell XPS13 computer running Ubuntu Desktop 20.04. The second-response delay $\Delta t_{53}$ is then sampled randomly many times, and for each trial 2500 measurements are collected to compute the average variance and frequency for that specific value of $\Delta t_{53}$. The results for two different values of $\Delta t_{32}$ are shown in Figures~\ref{fig:optimal_delay_metrics} and~\ref{fig:optimal_delay_metrics_1500}.

Given that this is a static experiment, $R_\mathrm{tot}$ essentially represents the uncertainty in the measurement obtained by averaging out all recorded measurements over a span of one second. Crucially, both experiments presented here seem to match the theoretical expectations quite well. As expected, the experiments with a longer $\Delta t_{32}$ have an order of magnitude higher standard deviation in the measurements, and in both experiments the standard deviation decreases as $\Delta t_{53}$ increases. The optimum $\Delta t_{53}$ seems to be somewhere around 1500 $\mu$s in the first experiment, and somewhere around 5000 $\mu$s in the experiment with longer $\Delta t_{32}$.

It is worth mentioning that there are some unmodelled phenomena in these results. Firstly, the reduction in frequency seems to occur in phases rather than the expected smooth curve, which is likely a consequence of the multi-processor nature of the computer as well as the scheduling of the implemented real-time scheduler. Additionally, there appears to be an unmodelled sinusoidal fluctuation with an amplitude proportional to the ratio $\f{\Delta t_{32}}{\Delta t_{53}}$. Nonetheless, these complexities further motivate the need to perform the aforementioned static experiment as a calibration step when utilizing TWR-based UWB ranging in any system. The theoretical optimal delay can be identified analytically and validated experimentally in order to ensure unmodelled system-specific phenomena are taken into consideration. 
